Probing and Fine-tuning Reading Comprehension Models for Few-shot Event Extraction

We study the problem of event extraction from text data, which requires both detecting target event types and their arguments. Typically, both the event detection and argument detection subtasks are formulated as supervised sequence labeling problems. We argue that the event extraction models so trained are inherently label-hungry, and can generalize poorly across domains and text genres.We propose a reading comprehension framework for event extraction.Specifically, we formulate event detection as a textual entailment prediction problem, and argument detection as a question answer-ing problem. By constructing proper query templates, our approach can effectively distill rich knowledge about tasks and label semantics from pretrained reading comprehension models. Moreover, our model can be fine-tuned with a small amount of data to boost its performance. Our experiment results show that our method performs strongly for zero-shot and few-shot event extraction, and it achieves state-of-the-art performance on the ACE 2005 benchmark when trained with full supervision.

==> approaches.tex <==
\section{Approaches}
\label{sec:approaches}

In this setting, we hope to investigate the ability of \bert model to predict events in a sentence without training. 
To this end, we attempt to convert event detection in the following 3 well-known problems: entailment prediction, question answering, and masked token prediction. 
\begin{enumerate}
    \item \textbf{Textual entailment (TE).}
        In standard textual entailment prediction setting, as depicted in ~\cite{mnli}, the model is given a pair of sentences, called ``premise'' and ``hypothesis'', and the model is tasked to predict whether the hypothesis is entailed by, contradicts to, or is irrelevant to the premise. 
        We convert event detection to this format by treating each sentence as the premise, and for each event, a statement that this event has occurred as the hypothesis. 
        Ideally, the model would classify that the sentence entails the event statement if the event indeed occurred in the context of the sentence. 
        
        We assume that the model predicts that the input sentence pair belongs to one of the three categories: \emph{contradictory}, \emph{entailment}, or \emph{neutral}. 
        Given a query-text pair constructed from Section~\ref{sec:preprocess:query_event} and ~\ref{sec:preprocess:query_argument}, we predict that the corresponding event or argument occurs if and only if the textual entailment model predicts ``entailment''. 
    \item \textbf{Question answering (QA).}
        The input in this setting includes a pair of sentences, ``question'' and ``text'', as described in ~\cite{rajpurkar2016squad}. The model is supposed to detect a span of words in the text that best answers the question, if there is any. 
        We have two type of questions: the ``Wh''-type and the Yes-No type, as described in Section~\ref{sec:method:arg_query}. We refer them as SQ-QA and PQ-QA, respectively. 
        For the first type, we apply the standard span detection approach. We treat the second type as a natural 0-1 classification problem, classifying the pair of sentences as either ``Yes'' or ``No''.
    \item \textbf{Masked token prediction. }
        This approach formulates event detection as a kind of ``fill in the blank''problem. 
        \bert is essentially a \emph{masked language model}, and it is supposed to predict masked tokens given the context. 
        We combine sentences with event queries, but instead of filling in actual event types, we place the special \texttt{[MASK]} token in place of event types and feed it to \bert. We then use \bert's pretrained weights to predict the most probable tokens on placeholders. 
        We propose this method mostly as a probing technique to understand what information about events \bert is able to summarize from texts and justify the performance of other models. 
\end{enumerate}

Throughout this paper, we used pretrained DistilBert model on relevant data and tasks for finetuning and evaluation. 
Specifically, for TE, we use DistilBert trained on MultiNLI~\cite{mnli} data~\footnote{https://huggingface.co/ishan/distilbert-base-uncased-mnli}. For both types of QA, we use DistilBert trained on SQuAD~\cite{rajpurkar2016squad} data~\footnote{https://huggingface.co/distilbert-base-cased-distilled-squad}. 

==> few_shot.tex <==
\section{Few-shot learning}
\label{sec:few_shot}
Since that unlike in many other tasks, pretrained language models does not significantly outperform random guessing as explained in Section~\ref{sec:zero_shot}, 
we naturally want to test the model's ability to transfer to event detection task with a few learning examples and if the model can build upon a few samples the link between model's semantic knowledge and the reasoning of events. 

Concretely, we experiment on TE and PQ-QA and see if the 
\newcommand{\tpm}{\(\pm\)}
\newcommand{\std}[1]{\((\pm#1)\)}

\begin{table*}[htbp]
    \centering
    \begin{tabular}{c|cccccc}
    \(K\)-shot & \(K=1\) & \(K=3\) & \(K=5\) & \(K=7\) & \(K=9\) & K=N\\  \hline
    \bert & & & & & \\
        TE & 43.02 \std{2.36} & 51.60 \std{2.15} & 51.51 \std{2.59} & 56.20 (\tpm 3.11)  & 56.83 (\tpm 4.36) & \\
        TE+D (1) & 23.10 (\tpm 5.20) & 45.94 (\tpm 4.80)  & 51.92 (\tpm 4.07) & 54.88 (\tpm 2.82) & 57.11 (\tpm 2.90) & \\
        TE+D (5) & 17.80 (\tpm 4.29) & 45.76 (\tpm 5.17) & 52.44 (\tpm 2.47) & 54.68 (\tpm 3.55) & 59.62 (\tpm 2.63) & \\
        PQ-QA & 40.23 \std{1.30} & 48.88 \std{3.27} & 50.05 \std{1.40} & 54.59 \std{1.88} & 55.77 \std{3.83} & \\
        PQ-QA+D (1) & 11.81 \std{13.45} & 47.86 \std{2.27} & 49.72 \std{4.57} & 52.89 \std{3.36} & 54.40 \std{4.41} & \\
        PQ-QA+D (5) & 6.34 \std{13.09} & 42.60 \std{3.01} & 49.34 \std{2.86} & 52.48 \std{3.79} & 54.97 \std{2.38} &
    \end{tabular}
    \caption{Results on few-shot learning. Here, we show the average micro F1-scores and standard deviations for each model and different number of training samples per class. TE and PQ-QA stand for textual entailment and polar-question question answering, +D means with event description, the number in the parenthesis means the maximum number of sentences in description. }
    \label{tab:few_shot_results}
\end{table*}

In Table~\ref{tab:few_shot_results}, we show few-shot learning results of different models with or without event description. 
Event descriptions in the annotation guide~\cite{ace05guide} can contain as many as 5 sentences, exceeding the text length of the sentence greatly. 
This makes harnessing the information in description hard when the number of training data is small. 
Therefore, in addition to training with full event descriptions, we truncate event descriptions to contain their the first sentences in hope of making the model easier to learn how to use information from descriptions. 

We make the following observations. 
First, when the training samples are too small (from \(K=1\) to \(K=5\)), adding event descriptions undermines model performance, especially in by a large margin when \(K=1\). 
Furthermore, when training with only the first sentence in description, the performance drop is much lower. 
However, when we have more samples per class, the models with event descriptions gradually outperform those without, and models with full descriptions outperform with only one sentence. 
Furthermore, when trained without descriptions, one observes counter-intuitively that the standard variance across multiple experiments increase with the number of samples. 

